G-TADOC: Enabling Efficient GPU-Based Text Analytics without Decompression

Text analytics directly on compression (TADOC) has proven to be a promising technology for big data analytics. GPUs are extremely popular accelerators for data analytics systems. Unfortunately, no work so far shows how to utilize GPUs to accelerate TADOC. We describe G-TADOC, the first framework that provides GPU-based text analytics directly on compression, effectively enabling efficient text analytics on GPUs without decompressing the input data. G-TADOC solves three major challenges. First, TADOC involves a large amount of dependencies, which makes it difficult to exploit massive parallelism on a GPU. We develop a novel fine-grained thread-level workload scheduling strategy for GPU threads, which partitions heavily-dependent loads adaptively in a fine-grained manner. Second, in developing G-TADOC, thousands of GPU threads writing to the same result buffer leads to inconsistency while directly using locks and atomic operations lead to large synchronization overheads. We develop a memory pool with thread-safe data structures on GPUs to handle such difficulties. Third, maintaining the sequence information among words is essential for lossless compression. We design a sequence-support strategy, which maintains high GPU parallelism while ensuring sequence information. Our experimental evaluations show that G-TADOC provides 31.1x average speedup compared to state-of-the-art TADOC.

==> challenge.tex <==
\section{Challenges}
\label{sec:challenge}

In this section,
we mainly discuss the challenges of enabling efficient text analytics on GPUs without decompression.

\vspace{\vsp{}}
\textbf{Challenge 1: GPU parallelism for TADOC}.
The high performance of GPU relies on the high throughput from thread-level parallelism.
First, as presented in~\cite{zhang2018efficient},
there exist massive dependencies among the DAG,
which leads TADOC difficult to be parallel.
Accordingly, TADOC utilizes coarse-grained parallelism that mainly processes different compressed files in parallel: each CPU thread handles a separate file~\cite{zhang2020tadoc}.
We cannot apply such coarse-grained parallelism on GPUs because a GPU supports thousands of threads and it is inefficient to split the compressed data into that large number of partitions.
Second,
If we use one GPU thread for one rule,
there is a workload unbalancing problem because the numbers of elements in different rules vary significantly.
GPUs launch threads in warp level, and the threads within a warp have to release resources simultaneously.
The workload imbalance problem decreases the parallelism degrees.
Third,
we cannot simply decide the number of threads for rules,
because of the various rule length.

\vspace{\vsp{}}


\textbf{Challenge 2: TADOC final result update conflict of massive GPU threads}.
The update conflict is a serious problem when we develop TADOC on GPUs.
First,
the update conflict of multiple threads writing to the same result buffer is not a serious problem on CPUs because the number of CPU threads is limited.
However,
on a GPU server,
when a large number of GPU threads write to the same result buffer,
we have to use atomic operations to guarantee correctness,
which incurs massive conflicts.
Second,
the complicated data structures used in TADOC cannot be applied in GPU environment.
For example, TADOC uses an \emph{unordered map} data structure for results such as word counts;
we need to develop our own similar data structures on GPUs with atomicity and consistency considered.
Third,
the amount of memory required by TADOC 
is unknown until runtime.
Even worse,
for TADOC on GPUs,
the memory sizes of different threads are also various,
which makes the update problem with thread conflicts more difficult.



\vspace{\vsp{}}



\textbf{Challenge 3: sequence maintenance of TADOC compressed data on GPUs}.
How to keep the sequence information on GPUs is also challenging.
Sequence maintenance is essential for sequence sensitive applications,
such as counting three continuous word sequences. 
First,
to keep the sequence information,
TADOC originally traverses the DAG in a DFS order~\cite{zhang2018efficient},
which is hard to be parallel.
Second,
a word sequence can span several rules and these rules could be controlled by different GPU threads.
Currently,
threads across different GPU blocks have no mechanism for synchronization.
Third,
TADOC uses \emph{map} data structures to store sequence counts.
For these sequence-based applications,
we need to develop special data structures in GPU memories to store sequences and  perform basic comparisons between threads.




